Towards Tight Convex Relaxations for Contact-Rich Manipulation

We present a novel method for global motion planning of robotic systems that interact with the environment through contacts. Our method directly handles the hybrid nature of such tasks using tools from convex optimization. We formulate the motion-planning problem as a shortest-path problem in a graph of convex sets, where a path in the graph corresponds to a contact sequence and a convex set models the quasi-static dynamics within a fixed contact mode. For each contact mode, we use semidefinite programming to relax the nonconvex dynamics that results from the simultaneous optimization of the object's pose, contact locations, and contact forces. The result is a tight convex relaxation of the overall planning problem, that can be efficiently solved and quickly rounded to find a feasible contact-rich trajectory. As an initial application for evaluating our method, we apply it on the task of planar pushing. Exhaustive experiments show that our convex-optimization method generates plans that are consistently within a small percentage of the global optimum, without relying on an initial guess, and that our method succeeds in finding trajectories where a state-of-the-art baseline for contact-rich planning usually fails. We demonstrate the quality of these plans on a real robotic system.

==> figures/DEPRECATED_experiments_and_plans.tex <==
%!TEX root = ../root.tex
\begin{figure*}[t]
	\centering
	\begin{subfigure}[b]{0.9\linewidth}
			\centering
			\includegraphics[width=\linewidth]{media/traj_14_plan.pdf}
    \end{subfigure}
	\begin{subfigure}[b]{0.9\linewidth}
			\centering
			\includegraphics[width=\linewidth]{media/traj_14_seq.png}
    \end{subfigure}
    
	\centering
	\begin{subfigure}[b]{0.9\linewidth}
			\centering
			\includegraphics[width=\linewidth]{media/traj_0_plan.pdf}
    \end{subfigure}
	\begin{subfigure}[b]{0.9\linewidth}
			\centering
			\includegraphics[width=\linewidth]{media/traj_0_seq.png}
    \end{subfigure}

   \caption{Our method is able to generate close-to globally optimal plans for pushing tasks with collision-free motion planning between contact modes. Here, two different pushing trajectories for a T-shaped slider are shown, stabilized with a feedback controller on a real robotic system.}
   \label{fig:experiments_and_plans}
\end{figure*}

==> figures/ablation_study.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{media/box_triangle_tee_ablation.pdf}
    \caption{Upper bounds on global optimality gap for 100 generated trajectories from randomly chosen boundary conditions plotted as a function of the total travelled rotation, for two different slider geometries.
    \smcomment{as discussed on Monday, i'm not sure you need this plot}
    }
    \label{fig:ablation_study}
\end{figure}

==> figures/contact_modes.tex <==
%!TEX root = ../root.tex

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{media/placeholder.png}
	\caption{
        TODO figure showing different contact modes
	}
	\label{fig:planar_pushing_model}
\end{figure}

==> figures/cost_effect.tex <==
\begin{figure}[h]
    \centering

    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/no_ang_vel_reg_trajectory.pdf}
        \caption{\(k_\omega=0\), \(k_f = 0\).}
        \label{fig:no_reg}
    \end{subfigure}
    \hfill %
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/ang_vel_reg_trajectory.pdf}
        \caption{\(k_\omega=1\), \(k_f = 0\).}
        \label{fig:ang_vel_reg}
    \end{subfigure}
    \hfill %
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/force_reg_trajectory.pdf}
        \caption{\(k_\omega=1\), \(k_f = 1\).}
    \end{subfigure}
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/comparing_violations_constraints.pdf}
        \caption{Violation of non-convex constraints~\eqref{eq:so2} and~\eqref{eq:slider_pusher_dynamics}.
}
        \label{fig:force_reg}
    \end{subfigure}
    
    \caption{Effect of the regularization term \(k_\omega\) and \(k_f\) on the tightness of the planned trajectories, evaluated by looking at constraint violations for the non-convex quadratic equality constraints in~\eqref{eq:so2} and~\eqref{eq:slider_pusher_dynamics}.
    \bpgcomment{TODO: Update equation numbers}}
    \label{fig:cost_effect}
\end{figure}

==> figures/evaluating_tightness.tex <==
%!TEX root = ../root.tex
\begin{figure}
    \centering
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/placeholder.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/placeholder.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/placeholder.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/placeholder.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/placeholder.png}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{media/placeholder.png}
    \end{subfigure}
    
    \caption{TODO Figures showing relaxation results before and after rounding
    }
    \label{fig:evaluating_tightness}
\end{figure}

==> figures/experiment_comparison.tex <==
%!TEX root = ../root.tex
\begin{figure*}[t]
	\centering
	\begin{subfigure}[b]{1.0\linewidth}
			\centering
			\includegraphics[width=\linewidth]{media/experiment_plan.pdf}
        \caption{Planned trajectory}
    \end{subfigure}
	\begin{subfigure}[b]{1.0\linewidth}
			\centering
			\includegraphics[width=\linewidth]{media/experiment_trajectory_1.pdf}
   \caption{Open-loop execution}
    \end{subfigure}
	\begin{subfigure}[b]{1.0\linewidth}
			\centering
			\includegraphics[width=\linewidth]{media/experiment_trajectory_1.pdf}
       \caption{Closed-loop execution}
    \end{subfigure}
    \caption{An example of a planned trajectory, open-loop execution of the plan, and stabilizing the plan with a feedback controller. \bpgcomment{TODO: Update video}}
    \label{fig:experiment_trajectory}
\end{figure*}
\begin{figure*}
        \centering
        \includegraphics[width=\textwidth]{media/experiments.pdf}
        \caption{Five different trajectories stabilized with feedback control. \bpgcomment{TODO: Update these with final videos.}}
        \label{fig:experiments}
\end{figure*}


==> figures/planar_pushing_all.tex <==
%!TEX root = ../root.tex
\begin{figure*}[ht]
    \begin{subfigure}[b]{0.32\linewidth}
    	\centering
    	%\includegraphics[width=\linewidth]{media/planar_pushing_kinematics.pdf}
            \input{figures/tikz_figures/pusher_slider/pusher_slider_kinematic_quantities}
        \caption{}
    	\label{fig:planar_pushing_kinematics}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        % \includegraphics[width=\linewidth]{media/planar_pushing_kinematics.pdf}
        \input{figures/tikz_figures/pusher_slider/pusher_slider_forces}
        \caption{}
        \label{fig:slider_pusher_forces}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\linewidth}
        \centering
        % \includegraphics[width=\linewidth]{media/planar_pushing_kinematics.pdf}
        \input{figures/tikz_figures/pusher_slider/pusher_slider_partitions}
        \caption{}
        \label{fig:slider_pusher_forces}
    \end{subfigure}
    \caption{\aacomment{What do we think of having all the "Slider" pictures as one figure? I can equalize the height and all that no problem.}}
\end{figure*}




==> figures/tikz_figures/pusher_slider/constants.tex <==
\pgfmathsetmacro{\rot}{35}
\pgfmathsetmacro{\AxisLength}{2}
\pgfmathsetmacro{\VecHeadLen}{3mm}
\pgfmathsetmacro{\VecHeadWidth}{2mm}
\pgfmathsetmacro{\trapleftangle}{60}
\pgfmathsetmacro{\traprightangle}{45}
\pgfmathsetmacro{\trapheight}{1.5cm}

==> figures/tikz_figures/pusher_slider/pusher_slider.tex <==
% Draw the slider
\input{figures/tikz_figures/pusher_slider/slider.tex}

% Label the origin of the pusher
\coordinate (SpP) at ($(S) + (-1.25,-0.2)$);
\fill[red!60] (SpP) circle [radius=0.2];
\fill[black] (SpP) circle [radius=0.05];
\draw[black, thick] (SpP) circle [radius=0.2];


==> figures/tikz_figures/pusher_slider/pusher_slider_forces.tex <==
\begin{tikzpicture}
  % Draw the pusher-slider
\input{figures/tikz_figures/pusher_slider/pusher_slider}
\input{figures/tikz_figures/pusher_slider/slider_frame}

  % Draw the forces
  \coordinate (F) at ($(SpP) + (0.2,-0.9)$);
  \node[above] at ($(SpP)!0.5!(F)$) {$f^{{}^{S}p^{P}}_{S}$};
  \draw[-{Stealth[length=\VecHeadLen, width=\VecHeadWidth]}] (SpP) -- (F) node[above] {};
  
\end{tikzpicture}

==> figures/tikz_figures/pusher_slider/pusher_slider_kinematic_quantities.tex <==
\begin{tikzpicture}
% Draw the pusher-slider
\input{figures/tikz_figures/pusher_slider/pusher_slider}

  % Label the origin
  \coordinate (W) at (-2,-2.3);
  \node[below left] at (W) {$W$};
  % Draw axis lines
  \draw[-latex] (W) -- ($(W) + (\AxisLength,0)$)node[right] {};
  \draw[-latex] (W) -- ($(W) + (0,\AxisLength)$) node[above] {};
    
  \input{figures/tikz_figures/pusher_slider/slider_frame}

  % Draw the angle measurement axis
  \draw[dashed] (S) -- (SxW) node[above] {};

  % Draw the vector WpS
  \draw[dashed,-{Stealth[length=\VecHeadLen, width=\VecHeadWidth]}] (W) -- (S) node[above] {};
  \node at ($(W)!0.5!(S) + (0,-0.7)$) {${}^{W}p^{S}$};
  
  % Draw the angle symbol
  \pic [draw, latex-latex, angle eccentricity=2, angle radius=0.7cm, "${}^{W}\theta^{S}$"]{angle=SxW--S--Sx};
  
  % Label the origin of the pusher
  \node[above] at ($(SpP)!0.5!(S) + (0, -0.1)$) {${}^{S}p^{P}$};
  \draw[dashed, -{Stealth[length=\VecHeadLen, width=\VecHeadWidth]}] (S) -- (SpP) node[above] {};
  
  
\end{tikzpicture}

==> figures/tikz_figures/pusher_slider/pusher_slider_partitions.tex <==
\begin{tikzpicture}
%   % Draw the pusher-slider
\input{figures/tikz_figures/pusher_slider/slider}

  % Get the corner coordinates
  \coordinate (topRight) at ($(slider.top right corner)$);
  \coordinate (topLeft) at ($(slider.top left corner)$);
  \coordinate (bottomLeft) at ($(slider.bottom left corner)$);
  \coordinate (bottomRight) at ($(slider.bottom right corner)$);

  \draw[dashed] (topRight) -- ($(topRight) + (90-\traprightangle*0.5+\rot:1)$) node {};
  \draw[dashed] (topLeft) -- ($(topLeft) + (90+0.5*\trapleftangle+\rot:1)$) node {};
  \draw[dashed] (bottomLeft) -- ($(bottomLeft) + (180+0.5*\trapleftangle+\rot:1)$) node {};
  \draw[dashed] (bottomRight) -- ($(bottomRight) + (-0.5*\traprightangle+\rot:1)$) node {};

  % Get the Center Face Coordinates
  \coordinate (topCenter) at ($(topRight)!0.5!(topLeft)$);
  \coordinate (leftCenter) at ($(topLeft)!0.5!(bottomLeft)$);
  \coordinate (bottomCenter) at ($(bottomLeft)!0.5!(bottomRight)$);
  \coordinate (rightCenter) at ($(bottomRight)!0.5!(topRight)$);

    % \node[below right] at (S) {$S$};
  % \node at ($(topCenter) + (\rot: 0.5)$) {$\mathcal{Q}_{1}$};
  \pgfmathsetmacro{\Qdist}{1.0}
  \node at ($(topCenter) + (90+\rot: \Qdist)$) {$\mathcal{Q}_{1}$};
  \node at ($(leftCenter) + (180+\rot: \Qdist)$) {$\mathcal{Q}_{2}$};
  \node at ($(bottomCenter) + (270+\rot: \Qdist)$) {$\mathcal{Q}_{3}$};
  \node at ($(rightCenter) + (\rot: \Qdist)$) {$\mathcal{Q}_{4}$};

  % Outline Slider in red
  \node [trapezium, trapezium left angle=\trapleftangle, trapezium right angle=\traprightangle, , minimum height=\trapheight, draw=red!40, line width = 1mm, text=black, rotate=\rot] (slider) at (S) {};
  \pgfmathsetmacro{\Cdist}{-0.2}
  \node at ($(topCenter) + (90+\rot: \Cdist)$) {$\mathcal{C}_{1}$};
  \node at ($(leftCenter) + (180+\rot: \Cdist)$) {$\mathcal{C}_{2}$};
  \node at ($(bottomCenter) + (270+\rot: \Cdist)$) {$\mathcal{C}_{3}$};
  \node at ($(rightCenter) + (\rot: \Cdist)$) {$\mathcal{C}_{4}$};


\end{tikzpicture}


==> figures/tikz_figures/pusher_slider/slider.tex <==
\input{figures/tikz_figures/pusher_slider/constants.tex}
% Draw the slider
\coordinate (S) at (0,0);
\node[below right] at (S) {$S$};
\node [trapezium, trapezium left angle=\trapleftangle, trapezium right angle=\traprightangle, , minimum height=\trapheight, fill=green!20, draw=black, text=black, rotate=\rot] (slider) at (S) {};


==> figures/tikz_figures/pusher_slider/slider_frame.tex <==
% Label the origin frame S
\coordinate (Sx) at ($(S) + (\rot:\AxisLength)$);
\coordinate (Sy) at ($(S) + (\rot+90:\AxisLength)$);
\coordinate (SxW) at ($(S) + (0:\AxisLength)$);
\node[below right] at (S) {$S$};
\fill (S) circle [radius=0.1];
% Draw axis lines for the frame S
\draw[-latex, rotate=\rot] (S) -- (Sx) node[right] {};
\draw[-latex, rotate=\rot] (S) -- (Sy) node[above] {};



==> figures/tikz_figures/transition_graph.tex <==
\begin{tikzpicture}
\pgfmathsetmacro{\nodesize}{0.5}
  % Draw vertices and edges for Q1 ... Q4
  \foreach \i in {1,2,3,4}
    \node[circle, draw, minimum size=\nodesize] (Q\i) at ({90*(\i)}:1) {$\mathcal{Q}_\i$};
  \foreach \i [evaluate=\i as \j using {int(mod(\i,4)+1)}] in {1,2,3,4}
    \draw[<->] (Q\i) -- (Q\j);

  % Draw vertices Ci and Cj, and connect to Q1 and Q3
  % \node[circle, draw, minimum size=\nodesize] (Ci) at ($(Q1)+(0,2)$) {$\mathcal{C}_{i}$};
  % \node[circle, draw, minimum size=\nodesize] (Cj) at ($(Q3)+(0,-2)$) {$\mathcal{C}_{j}$};
  % \draw[<->] (Ci) -- (Q1) (Cj) -- (Q3);

  % Draw vertices and edges for C1 ... C4
  \foreach \i in {1,2,3,4}
    \node[circle, draw, minimum size=\nodesize] (C\i) at ($(Q\i)+({90*(\i)}:2)$) {$\mathcal{C}_\i$};
  \foreach \i [evaluate=\i as \j using {int(mod(\i,4)+1)}] in {1,2,3,4} {
    \draw[<->] (C\i) -- (C\j);
    \draw[<->] (C\i) -- (Q\i);
}
 
\end{tikzpicture}


==> sections/decrecated_vol_1/introduction.tex <==
%!TEX root = ../root.tex

\tmcomment{I would be a little more bold in the first two paragraphs of the intro. I would start by speaking about optimal control through contact in general: why it's important and why it's hard to solve (discrete + continuous). Then I would say that there are no good ways to reason about contact planning globally. (You can cite, among many other works, Mike Posa's IJRR paper and Twan Koolen's thesis.) Then I would introduce the GCS idea, and say something like what you said in the abstract (vertices are contact modes and convex sets are SDP relaxations of QS dynamics). Here it's important to stress and give an intuition of how GCS+SDP is more than its parts combined (most people think of graphs as tools that allow brute force enumeration, here we use to give structure to the optimization problem--most people are surprised when you tell them that you can solve an SPP with convex opt). Finally, I would say that we start from a simple problem that is planar pushing. I would not try to convince the reader that planar pushing is really an important problem in practice?}
 
Planar pushing is an essential task in scenarios ranging from warehouse automation to service robotics, and is among the simplest examples of non-prehensile manipulation tasks.
Yet, current state-of-the-art robotics approaches struggle with solving planar pushing to optimality, as the problem represents many of the key challenges with robotic manipulation such as hybrid dynamics and underactuation.

Today, this problem is typically solved with imitation learning \cite{chiDiffusionPolicyVisuomotor2023a}, or in two steps with a sampling-based method \cite{chengContactModeGuided2021a,chengContactModeGuided2022,pangGlobalPlanningContactRich2022,chavandafleInHandManipulationMotion2018}, or a local motion planning method \cite{doshiHybridDifferentialDynamic2020,lefebvreDifferentialFlatnessSliderPusher2023,zhouPushingRevisitedDifferential2019}, combined with a model-based control approach \cite{hoganReactivePlanarNonprehensile2020,hoganFeedbackControlPusherSlider2020}.
Imitation-learning approaches demonstrate several impressive characteristics, such as output feedback and robustness to disturbances. However, they require demonstrations for training, which currently is an expensive data-gathering process executed by human operators.
In principle, one can envision an imitation learning pipeline where a combination of model-based motion planning and control method provides optimal demonstrations, which are used to train a learned policy with the desirable characteristics as mentioned above.
However, current motion-planning techniques are not well suited for such a pipeline: Sampling-based motion planning has the drawback of randomized plans, whereas local motion planning gets stuck in local minima.
This motivates the search for a model-based motion planning algorithm which can provide globally optimal motion plans.

%\todo{Motivational paragraph:} Planar pushing is an essential task for automation in scenarios ranging from industrial assembly to service robotics. Etc Etc. TODO. Planar pushing is a fundamental task bla bla.
%One of the simplest non-prehensile manipulation tasks, yet hard to plan for etc. Hybrid dynamics and underactiation. Robots being far behind humans etc. Planar pushing is a canonical manipulation skill which represents many of the key challenges with robotic manipulation: hybrid dynamics, underaction.

In this work, we present a novel motion planning framework for contact-rich manipulation tasks based on convex optimization. We formulate the motion planning problem as a \acrfull*{spp} in a \acrfull*{gcs}, a class of \acrfull*{micp} problems which often can be solved efficiently to global optimality through a tight convex relaxation \cite{marcucciShortestPathsGraphs2022}. \tmcomment{I would not say that the SPP in GCS is a class of MICP. The SPP in GCS is a problem that you can formulate independently of MICP, then, if you like, you can use MICP to solve it.} In our formulation, a path in the graph corresponds to a mode sequence, and the convex sets represent contact manifolds. By solving the \acrshort*{spp} in \acrshort*{gcs} problem, we are thus able to simultaneously search for the optimal mode sequence and the optimal motion within each mode.

In contrast to prior work, we seek to simultaneously optimize over contact locations \bpgcomment{double verify that there are no other works doing this}, contact forces, and object poses. Because of this, the contact manifolds and quasi-static dynamics are described by nonlinear constraints, which we formulate as the feasible set of a non-convex \acrfull*{qcqp}. To tackle the non-convexities, we will use semidefinite relaxations to relax the non-convex \acrshort*{qcqp} into a \acrfull*{sdp}, which can be solved efficiently.

\bpgcomment{We should also mention how quasi-static contact modes go hand in hand with GCS somewhere}

\tmcomment{Overall, try to better convey the big picture. This is the first approach that tackles control through contact globally in an elegant way. We are able to elegantly blend the discrete logic and the continuous dynamics of control through contact into a convex optimization problem. It's the first work that can use continuous (convex!) optimization to think about mode switches. Previous approaches to the problem used either local (sampling or NLP) or MINLP+B\&B (which is global but in a fake way, since B\&B resorts to exhaustive enumeration). Then you can add a sentence to say the limitations of the approaches, and clarify that we don't think that control throguh contact is solved just bcs our approach can do planar pushing...}

\textbf{Contributions}
Our first contribution is a formulation of the motion planning problem for quasi-static contact within a fixed mode where one simultaneously searches over the object poses, contact locations, and contact forces as a (non-convex) \acrshort*{qcqp}, for which the convex \acrshort{sdp} relaxation is empirically tight for many problem instances.
\bpgcomment{specify when and why the relaxation is not tight.}
Next, using the \acrshort*{sdp} relaxation for each contact mode under consideration, we are able to formulate the motion planning problem as a \acrshort*{spp} in a \acrshort*{gcs}, allowing us to simultaneously search for the optimal mode sequence and the motion within each mode.


\textbf{Paper structure}
This paper is organized as follows: In \cref{sec:related_work}, we give an overview over related litterature, providing a clear comparison of our approach to existing methods in the field.
Then, a high-level description of the problem statement and our approach to solving the problem is presented in \cref{sec:problem_statement}.
We provide the reader with the necessary mathematical background material in \cref{sec:technical_background}, before we review the formulation of the pusher-slider system and its quasi-static dynamics in  \cref{sec:mechanics_of_planar_pushing}. Then, in \cref{sec:motion_planning} we present our core contribution which is the motion planning method.
Finally, we present our experimental results in \cref{sec:experiments}, where we execute the generated motion plans on a real system. Conclusions and future work are covered in \cref{sec:conclusion}

==> sections/deprecated_vol_0/planning_formulation.tex <==

\subsection{Formulating the Contact Problem with \acrshort{gcs}}
\label{sec:gcs_contact_planning}

In this section, the different pieces from \cref{sec:gcs}, \cref{sec:sdp_relaxation_of_qcqp}, and \cref{sec:mechanics_of_planar_pushing} will be combined to formulate a motion planning algorithm for the hybrid planar pushing system presented in \cref{sec:mechanics_of_planar_pushing}. The main approach to the motion planning problem will be to build a graph $G = (\mathcal{V}, \mathcal{E})$ that can be solved with \acrshort{gcs}, where each vertex $v \in \mathcal{V}$ corresponds to a mode of the hybrid system, with an edge $e = (u,v)$ for all possible mode transitions.

\bpgcomment{Here I first present the "continuous" version, then later I discretize it, because I worry that the knot point indices etc will clutter up the notation a lot. I am beginning to think that this perhaps is a bad way of doing it, and that directly presenting the discretized version would be better. Some feedback here would be good!}

We are now considering the planar pushing system in its full generality, including when there is no contact between the pusher and slider. We will assume an ellipsoidal pusher with the main axis parallel with the $z$-axis, which means there is only going to be one contact point ($N_c = 1$).
Let the planar position of the \acrshort{com} of the pusher in the world frame be $\prescript{W}{}{p}^P \in \R^2$, where the quasi-static assumption gives $\prescript{W}{}{v}^P = \frac{d}{dt} \prescript{W}{}{p}^P \approx 0$. Following \cref{sec:mechanics_of_planar_pushing}, the full configuration of the quasi-static planar pushing system (independent of the contact mode) at a given time is then fully described by the vector $(\prescript{W}{}{p}^B, \prescript{W}{}{\theta}^B, \prescript{W}{}{t}^B, f^c_W, \prescript{W}{}{p}^P) \in \R^{10}$.

We will define a planar pushing task by an initial and final planar pose for the slider and a planar position for the pusher, denoted as the configurations $(\prescript{W}{}{p}^B, \prescript{W}{}{\theta}^B, \prescript{W}{}{p}^P)_\sigma \in \R^5$ and $(\prescript{W}{}{p}^B, \prescript{W}{}{\theta}^B, \prescript{W}{}{p}^P)_\tau \in \R^5$, respectively. These conditions will be added as singleton sets in the graph $G$. A valid motion plan is a plan that continuously changes the slider and pusher poses from the initial to the target configuration while adhering to the constraints presented in \cref{sec:mechanics_of_planar_pushing} and while avoiding penetration between the pusher and the slider. Such a plan will necessarily consist of both contact modes where the pusher is in contact with the slider and where there is no contact.

First, the different modes and their corresponding vertices with convex sets will be introduced in \cref{sec:in_contact_vertices} and \cref{sec:collision_free_vertices}. Then, to implement and solve the optimization problem, we will show how the system is discretized in \cref{sec:discretization}. Finally, \cref{sec:retrieving_a_traj} will cover how a feasible trajectory is retrieved at the end of the motion planning algorithm.

\subsubsection{In-Contact Vertices}
\label{sec:in_contact_vertices}
When the pusher is in contact with the slider, the dynamics of the system are modelled with the formulation from \cref{sec:mechanics_of_planar_pushing}. For a particular contact mode, let the set defined by the friction cone constraints in \cref{eq:friction_cone}, the mode constraints in \cref{eq:mode_sticking,eq:mode_sliding_left,eq:mode_sliding_right} and the quasi-static dynamics in \cref{eq:quasi_static_dynamics} be denoted as $\mathcal{C}$. By introducing the auxiliary variables $c_\theta := \cos{(\prescript{W}{}{\theta}^B)}$ and $c_\theta := \sin{(\prescript{W}{}{\theta}^B)}$ and substituting the trigonometric terms, with the additional constraint $c_\theta^2 + s_\theta^2 = 1$, the quasi-static dynamics in \cref{eq:quasi_static_dynamics} can be represented by quadratic equality constraints. The set $\mathcal{C}$ is then described by affine constraints and quadratic equality constraints, meaning that it can be described as the feasible set of the \acrshort{qcqp} shown in \cref{eq:qcqp}. Following the result from \cref{th:convex_outer_approximation}, we can use the \acrshort{sdr} presented in \cref{eq:qcqp_relaxation} to form the convex outer-approximation $\mathcal{C}_{\text{relax}} \supseteq \mathcal{C}$.

For each contact mode of the hybrid system, we will add a vertex $v$ with a corresponding spectrahedral set $\mathcal{C_\text{relax}}$ to the graph $G$. The choice of cost function is crucial for the tightness of the \acrshort{sdr}. In this work, we choose action of the slider over the trajectory as the vertex cost $l_v$, defined as:
\begin{align}
    A &= \int_0^T \left[ \frac{1}{2}m \norm{\prescript{W}{}{v}^B(t)}^2 + \frac{1}{2} I \norm{\prescript{W}{}{\omega}^B (t)}^2 \right] dt
    \label{eq:in_contact_cost}
\end{align}
\todo{Verify that we are actually minimizing action, or reformulate this part.}
where the squared angular velocity $\norm{\omega}^2$ associated to a rotation described by the matrix $R \in SO(3)$ can be retrieved as:
\begin{align}
\lVert \omega \rVert ^2 =
\omega ^\intercal \omega
&= 
\frac{1}{2}
\text{Tr}([\omega]^\times {}^\intercal [\omega]^\times)
= \frac{1}{2} \text{Tr}(\dot R^\intercal \dot R) \nonumber \\
&=
\frac{1}{2} \text{vec}(\dot R)^\intercal
\text{vec}(\dot R) \nonumber
:= \frac{1}{2} \lVert \dot r \rVert^2
\end{align}
where $\text{vec}(\cdot)$ denotes the stacking of columns of a matrix into a vector, and identities $[\omega]^\times = \dot R R ^ \intercal$ , $\frac{1}{2} \text{Tr}([a]^\times {}^\intercal [a]^\times)
=
\text{vec}(a)^\intercal
\text{vec}(a)
= a^\intercal a$, and
$\text{Tr}(A^\intercal B)
=
\text{vec}(A)^\intercal
\text{vec}(B)$
have been used.

Empirically, when combined with the discretization in \cref{sec:discretization}, the cost function in \cref{eq:in_contact_cost} yields tight solutions for the rotational parameters $c_\theta$ and $s_\theta$, for all cases except when the difference between the initial and target configuration is exactly $\pi$ radians.

\todo{Change this part if we can prove tightness for simple problems.}


\subsubsection{Collision-Free Vertices}
\label{sec:collision_free_vertices}
When the pusher is not making contact with the slider and under the quasi-static assumptions, one must have $f^c_B = 0$, $\prescript{W}{}{t}^B = 0$. Hence, for the vertices that represent modes where there is no contact, we only consider the variables $(\prescript{W}{}{p}^B, \prescript{W}{}{\theta}^B, \prescript{B}{}{p}^P) \in \R^5$. Notice that the position of the pusher is measured and represented in the body frame $B$. In these coordinates, the total non-convex space of collision free configurations can be decomposed into several polyhedral sets, each which will correspond to its own vertex $v$ in the graph $G$. For each such vertex $v$, the convex set $\mathcal{N}$ corresponding to a collision-free region will simply be defined by 
\begin{align}
    \mathcal{N} = \set{
        \prescript{B}{}{p}^P \mid 
        A \prescript{B}{}{p}^P \geq b
    }
\end{align}
where $A$ and $b$ represent the hyperplanes that define the collision-free region in the body frame $B$. A decomposition into such sets is shown in \cref{fig:collision_free_regions}

\input{figures/collision_free_regions}

For a vertex $v$ corresponding to a non-collision mode of the system, we will minimize squared Euclidean distance over the pusher trajectory, while maximizing the distance to the slider. The cost of vertex $v$ is thus defined as:
\begin{align}
    \int_0^T \left[ \norm{\prescript{B}{}{p}^P(t)}^2_2 - \frac{1}{a^\intercal \prescript{B}{}{p}^P + b} \right] dt
    \label{eq:collision_free_cost}
\end{align}
where $(a,b) \in \R^3$ represent the hyperplane corresponding to the particular contact face for the collision-free region.

\todo{Right now we don't actually use the SOCP cost, this needs to be implemented!}

\subsubsection{Discretization of the dynamics}
: % TODO: remove

\bpgcomment{I am not sure if it makes sense to have this as its own part, of the cost functions etc. should already be presented as discretized in the previous subsections.}

\label{sec:discretization}
In order to implement and solve the \acrshort{gcs} optimization problem, we need to pick a representation for the trajectories. In this work, we will discretize time and represent the trajectories by discrete knot points, using piecewise linear interpolation between the knot points. In particular, let $\Delta t$ denote a fixed timestep, and for a given quantity $x$, let $x[n] := x(n \Delta t)$ denote the value of $x$ at knot point $n$. 


Representing the trajectories by discrete knot points means that the dimension of the convex sets associated with the vertices in the graph $G$ will grow as the number of knot points grows. For instance, if a vertex $v$ for one knot point is associated with a point $x_v \in \mathcal{X}^v \subset \R^m$, then allowing $n$ knot points in this set will require associating $v$ with a point $\bar x_v \in \bar{\mathcal{X}}_v = \mathcal{X}_v^n \subset \R^{n m}$ (where $(\cdot)^n$ denotes the $n$-ary Cartesian power).

Using this trajectory representation, we can approximate the cost functions for both the contact vertices and the non-collision vertices. For the contact vertices, the cost function in \cref{eq:in_contact_cost} and quasi-static dynamics in \cref{eq:quasi_static_dynamics} involve the derivatives for certain variables. For a given vector $x$, we will use forward finite differences to compute derivatives:
\begin{align}
    \dot x[n] = \frac{x[n+1] - x[n]}{\Delta t}
\end{align}
This gives the following discrete approximation of the cost function in \cref{eq:in_contact_cost} (where the frames have been dropped to improve readability):
\begin{align}
A &= \int_0^T \left[ \frac{1}{2}m \lVert v (t) \rVert ^2 + \frac{1}{2} I \lVert \omega(t) \rVert^2 \right] dt \nonumber \\
&= \int_0^T \left[ \frac{1}{2}m \dot p(t)^\intercal \dot p(t) + \frac{1}{4} I \dot r(t)^\intercal \dot r(t) \right] dt \nonumber \\
&\approx
\sum_{k=0}^{N}
k_v
\lVert p[k+1] - p[k] \rVert^2
+
k_\omega
\lVert r[k+1] - r[k] \rVert^2
\label{eq:in_contact_cost_discrete}
\end{align}
for suitable constants $k_v$ and $k_\omega$, and $r[k] = \text{vec}(R)$. We note that under the chosen formulation and discretization, minizing the cost in \cref{eq:in_contact_cost} in fact corresponds exactly to minimizing the squared Euclidean distance in the position and rotation parameters, as is clearly seen in \cref{eq:in_contact_cost_discrete}

For the non-collision vertices defined in \cref{sec:collision_free_vertices}, the cost is simpler:
\begin{align}
    \sum_{k=0}^{N}
    \lVert p_{k+1} - p_{k} \rVert^2 + \text{TODO: SOCP cost}
\end{align}
\bpg{Here I don't feel that it makes sense to first present the continuous cost, then the discrete one.}

\todo{We actually use slerp for rotations, this must be mentioned somewhere.}

\subsubsection{Building the Graph}
\todo{Continuity constraints are enforced like bla bla}
\label{sec:retrieving_a_traj}

\subsection{Tightening Constraints and Body Frame Formulation}
\todo{Write down how we use the quantities in the body frame}
\todo{Add a paragraph on the redundant tightnening constraints that we add}

==> sections/deprecated_vol_2/old_introduction.tex <==
%!TEX root = ../root.tex

Optimal planning and control through contact is an important and challenging problem in robotics, and includes tasks like robot locomotion
It generally involves both a hybrid and underactuated dynamical system, making planning and control difficult.
Although there are several existing methods for tackling the problem, there is generally a lack of a method which can reason globally about these problems.
While local methods can generate impressive motion plans for many tasks, they can be unreliable and inherently lack an abilility to do global reasoning.
On the other hand, methods that attempt global planning typically only works for small systems, and suffers from poor scalability.
%\bpgcomment{Writing is not good I know but is the intro structure + literature review structure good now? If so I will fix the language/phrasing.} \rtcomment{It seems a bit inconsistent with the title. You say "towards global" in the title, but it sounds like global was already a state-of-the-art here.}
%\smcomment{There isn't a method out there that would give us optimal / near optimal trajectories through contact. Two years ago Russ couldn't give a diffusion intern optimal T-pushing trajectories. We can now. I think a stronger (also accurate) point is that global methods for planning through contact barely exist. Local methods can't plan through complex contact switch sequences. LGP by Toussaint doesn't reason about contact (rather about kinematic switches), other methods like PDDLStream are sampling based; both reason globally, but you can't guarantee optimality / optimality bounds.}

%\smcomment{make it clear what gap you are talking about; if the gaps is combinatorics + continuous decision making, then that's GCS, not this paper. address inability to plan near optimal trajectories through contact?}
In this work, we address this gap by presenting a novel motion planning framework for non-prehensile manipulation that naturally blends the discrete logic and continuous dynamics of global planning through contact into a convex optimization problem. 
We formulate the global motion planning problem as a \acrfull*{spp} in a \acrfull*{gcs}, a class of optimization problems which can often be solved efficiently to global optimality~\cite{marcucci2023shortest}.
In our formulation, a path in the graph corresponds to a contact sequence, and the convex sets represent quasi-static contact dynamics within a fixed mode for the system.
Because we simultaneously optimize over the object pose, contact locations and contact forces, the sets of feasible quasi-static trajectories are non-convex, and we outer-approximate them as convex sets using \acrfull*{sdp} relaxations.
In particular, we present a convex relaxation of the (non-convex) bilinearities appearing in the motion planning problem that is often surprisingly tight.
This is in contrast to other related works
where one has to resort to higher-order \acrshort*{sdp} relaxations
\bpgcomment{cite Ram Vasudevan},
which would be computationally intractable for the problems considered in this work.
%\rtcomment{I think you should make it more clear that one of the contributions of the paper is that you're presenting a convex formulation of the bilinearities appearing in this problem which is often surprisingly tight using only the first-order relexation. (for instance, we can cite recent work by Ram V et al at Michigan which claim things are tight, but require higher-order relaxations. I remember my conversation with Zac Manchester who said something that he had less of a grasp of than we do, but said it like this "it turns out multibody dynamics is convex". That's too much, but let's not be too understated.}
%\smcomment{+1 on making it clear that deriving the SDP relaxation is a contribution. i don't think many robotics people are aware that you can write nice pretty-tight convex relaxations of rotations like that}
We show empirically that the convex relaxation is sufficiently tight that a simple, cheap rounding step obtains near-global solutions 
Additionally, the graph structure of \acrshort*{gcs} allows us to also encode collision-free motion planning between contact modes, by partitioning the collision-free subset of the configuration space into convex sets that are added to the graph.
In summary, by solving the \acrshort*{spp} in \acrshort*{gcs} problem, we are thus able to simultaneously search for the optimal contact sequence, the optimal motion within each contact mode, and a collision-free path between the contact modes.

\input{figures/experimental_setup}

As a first step towards global motion planning through contact, in this work we explore the task of planar pushing, first studied by Mason in~\cite{masonMechanicsPlanningManipulator1986}. Planar pushing has applications that span from warehouse automation to service robotics, and 
although it is among the simplest examples of non-prehensile manipulation, current state-of-the-art approaches are still unable to solve this problem reliably to global optimality.
The method proposed in this paper can simultaneously reason about the high-level discrete mode switches and the low-level continuous dynamics of planar pushing.
In addition, by being based on convex optimization, our approach can reliably solve these contact-rich problems globally.
%\tmcomment{I've rewritten the paragraph. LMK if you guys like it better. (Old version commented below.)}
% As a first step towards global motion planning through contact, in this work we explore the task of planar pushing, first studied by Mason in~\cite{masonMechanicsPlanningManipulator1986}.
% Planar pushing has applications that span from warehouse automation to service robotics.
% While it is among the simplest examples of non-prehensile manipulation tasks, current state-of-the-art approaches struggle with planning globally optimal planar pushing trajectories.
% We show that our method is able to generate globally optimal motion plans for this problem, and note that 
% this is the first work able to use convex optimization to simultaneously reason about the global mode switches and the continuous motion for a planning problem for a contact-rich task.
%\aacomment{Technically not true. See Lu's work that did it with SOS ;)} \rtcomment{Lu's work used a coarse teleportation version of contact; it could not generate the plans that we generate here.} \bpgcomment{How should I change sentence?}.
%\smcomment{there is also Simon + Taylor's work on optimization using optimization based dynamics, and hybrid DDP / DDP with LCP constraints. all three could discover new contact modes, albeit in a local fashion. may be just don't make "we be first" statement?}
The runtimes of our method increase quickly but still polynomially with the number of contact modes, as opposed to the exponential complexity of a naive enumeration of all the possible mode sequences.
%While our method scales with the number of contact modes in the system, it scales much better than performing exhaustive contact sequence enumeration.
%\tmcomment{I don't love this sentence. ``Scaling'' on its own doesn't mean much. I'd rather say something like ``The runtimes of our method increase quickly but still polynomially with the number of contact modes, as opposed to the exponential complexity of a naive enumeration of all the possible mode sequeneces.''}
We emphasize that, while in this paper we focus on planar pushing, the techniques we introduce generalize to more complex contact-rich problems.
%We emphasize that while the application of our method in this work is planar pushing, our main motivation is a method that generalizes to general contact-rich tasks.
%\tmcomment{This is also strange: the real question is if our method goes beyond planar pushing, not really what is our main motivation. So I would either remove this sentence or say ``We emphasize that, while in this paper we focus on planar pushing, the technicques we introduce generalize to more complex contact-rich problems.`}

%\paragraph{Contributions}
%Our first contribution is a formulation of the motion planning problem for quasi-static contact within a fixed mode where one simultaneously searches over the object poses, contact locations, and contact forces as a (non-convex) \acrfull*{qcqp},
%for which the convex \acrshort{sdp} relaxation yields high-quality solutions that can often be rounded using a cheap rounding step to retrieve a globally optimal solution.
%Next, employing the \acrshort*{sdp} relaxation for the contact modes of the system, we are able to formulate the global motion planning problem as a \acrshort*{spp} in a \acrshort*{gcs}, allowing us to simultaneously search for the optimal contact sequence, the trajectory in each contact mode, and the collision-free motion between contacts.
%\tmcomment{It's nice to have the contributions spelled out, but if we need space I think this can be cut or blended with the text above?}
%\aacomment{I agree. If anything the intro repeats the same point one too many times and could be best summarized using basically this paragraph.}

%\rtcomment{I could see writing a little more in the paper (intro?) about the potential generality of the approach to complete the motivation.  Or possibly flipping the motivation to go against the standard advice... I think it could be fair to say "We want to see if GCS can handle planning through contact, so we explore it deeply on planar pushing".}

%\paragraph{Paper structure}
%This paper is organized as follows: In \Cref{sec:related_work}, we give an overview of the related literature, providing a clear comparison of our approach to existing methods in the field.
%Then, in \Cref{sec:problem_statement} we state the planning problem analyzed in this paper, and present our approach to solving the problem in high-level terms in \Cref{sec:high_level_approach}.
%We provide the reader with the necessary mathematical background material in \Cref{sec:technical_background}, before we review the formulation of the pusher-slider system and its quasi-static dynamics in  \Cref{sec:mechanics_of_planar_pushing}. Then, in \Cref{sec:motion_planning} we present our core contribution which is the motion planning method.
%Finally, we present our experimental results in \Cref{sec:experiments}, where we execute the generated motion plans on a real system. Conclusions and future work are covered in \Cref{sec:conclusion}
%
%\tmcomment{I would be a little more bold in the first two paragraphs of the intro. I would start by speaking about optimal control through contact in general: why it's important and why it's hard to solve (discrete + continuous). Then I would say that there are no good ways to reason about contact planning globally. (You can cite, among many other works, Mike Posa's IJRR paper and Twan Koolen's thesis.) Then I would introduce the GCS idea, and say something like what you said in the abstract (vertices are contact modes and convex sets are SDP relaxations of QS dynamics). Here it's important to stress and give an intuition of how GCS+SDP is more than its parts combined (most people think of graphs as tools that allow brute force enumeration, here we use to give structure to the optimization problem--most people are surprised when you tell them that you can solve an SPP with convex opt). Finally, I would say that we start from a simple problem that is planar pushing. I would not try to convince the reader that planar pushing is really an important problem in practice?}

%\tmcomment{Overall, try to better convey the big picture. This is the first approach that tackles control through contact globally in an elegant way. We are able to elegantly blend the discrete logic and the continuous dynamics of control through contact into a convex optimization problem. It's the first work that can use continuous (convex!) optimization to think about mode switches. Previous approaches to the problem used either local (sampling or NLP) or MINLP+B\&B (which is global but in a fake way, since B\&B resorts to exhaustive enumeration). Then you can add a sentence to say the limitations of the approaches, and clarify that we don't think that control throguh contact is solved just bcs our approach can do planar pushing...}

==> sections/deprecated_vol_2/old_related_work.tex <==
%!TEX root = ../root.tex

%\subsection{Control through contact}

\bpgcomment{Focus here has been getting the structure right. For this whole section: Improve language, add more references.}

A common approach to control and planning through contact is optimal control, and many of these methods are local and use \acrfull*{nlp}. 
Methods based on trajectory optimization have successfully been applied to a variety of tasks like planning for locomotion~\cite{kuindersma2016optimization}, acrobatic tasks for humanoids~\cite{mordatch2012discovery,tassa2012synthesis}, or planar pushing~\cite{doshiHybridDifferentialDynamic2020}.
Contact-implicit methods have successfully been applied to locomotion planning for a variety of different robotics systems~\cite{manchester2020variational,posaDirectMethodTrajectory2014}, as well as to non-prehensile manipulation tasks~\cite{jinTaskDrivenHybridModel2022,wangContactImplicitPlanningControl2023}.
While these methods have shown the ability to generate incredible motion plans for many tasks, they can be unreliable and lack the ability to do global reasoning.
\smcomment{so, what about DDP with LCP constraints and Simon/Taylor's traj opt with op based dynamics? in principle they enumerate all contact modes and have all contact modes always active, hence should be able to discover arbitrary mode sequences; does this count as global? I'd ask Terry.}

On the other hand, many existing methods for planning through contact are sampling-based.
Existing methods that either enumerate contact modes to guide the search have been employed for a variety of different non-prehensile tasks~\cite{chengContactModeGuided2021a,chengContactModeGuided2022}, or methods that use smoothed contact models to avoid reasoning explicitly about the contact modes have been employed to plan for dexterous hands and other contact-right manipulation~\cite{pangGlobalPlanningContactRich2022}.
\bpgcomment{Add \cite{chavan-dafle2020planar} that use sampling-based methods to sample configurations on the motion cone}
These methods are often in some sense more global than the methods based on \acrshort*{nlp}, and can reason about tasks at a more global level. However, sampling on constraint-manifolds is hard and seems unatural.
 
Another common approach is \acrfull*{rl} or \acrfull*{bc} methods. \acrshort*{rl} methods have been applied to a variety of manipulation tasks in simulation~\cite{lillicrap2015continuous,rajeswaran2017learning} simple tasks in the real world~\cite{gu2017deep}, and more recently has shown success for real-world dexteruous hands~\cite{andrychowicz2020learning,chen2022system,qi2023general,yin2023rotating} and impressive robustness for quadruped locomotion~\cite{hwangbo2019learning}. Recent work has also been done on automatically shaping a reward function~\cite{ma2023eureka}. \acrshort*{bc} methods have been succesfully applied to a variety of manipulation tasks like planar pushing~\cite{florence2022implicit,chi2023diffusion}. Learning-based approaches are generalizable as they require no knowledge of the model, but usually requires expensive training, a user-shaped reward function, or expert demonstrations which can be expensive to generate. \rtcomment{I would not be surprised if our longer-term solution used learning to address the lowest-level combinatorial problem (e.g. for a dexterous hand). Maybe we can add an extremely speculative sentence about that here? I'd prefer to not give the impression that it's learning \emph{or} GCS.}

There are also methods that attempt global planning and control through \acrfull*{mip}.
Globally optimal plans can be achieved through the use of spatial \acrfull*{bb} methods, where the non-convex search space is partioned into smaller subsets and the problem is solved through exhaustive enumeration, which has been succesfully applied to locomotion~\cite{koolenBalanceControlLocomotion2020} and manipulation tasks~\cite{aceituno-cabezasGlobalQuasiDynamicModel2020}. 
Another approach is linearization to obtain a \acrfull*{pwa} system and employing \acrshort*{mip} methods~\cite{marcucci2019mixed}, which has been applied to push-recovery~\cite{marcucci2017approximate},
general manipulation tasks \cite{aceituno2017simultaneous,aydinoglu2022real}, and planar pushing~\cite{hoganReactivePlanarNonprehensile2020}. \acrshort*{mip}-based methods have also been employed in combination with learning, for planar pushing with a learned mode-scheduler~\cite{hoganReactivePlanarNonprehensile2020} or with learned \acrshort*{pwa} dynamics in~\cite{liu2023model}.
While \acrshort*{mip} methods have shown success for relatively simple tasks, they suffer from poor scalability and struggle with nonlinearities arising from rotations and cross-products between contact points and forces.\rtcomment{I think you are saying the right things, but perhaps missing the emphasis I would expect? the specific way that previous approaches struggled is by making a combinatorial piecewise approximation of the rotations; we use the SDP relaxations and show that they are tight.}
\smcomment{The way i see it, there are two relaxations happening here: discrete choices and rotation. In discrete perspective, most methods used big M integer relaxations(correct me Tobia if that's false), which are terribly lose; perspective machinery of gcs fixed that. for rotations, people discretized rotations or used mccormic envelopes. Your relaxation is more precise + tighter. I'd imagine you should put emphasis on both these things in discussing MICP literature}
Yet another approach is to leverage convex relaxations of the nonlinear dynamics, in combination with \acrshort*{mip} which has been applied to locomotion in ~\cite{ponton2016convex}.

Our method is closer to the last category of \acrshort*{mip}, but is more efficient.
We employ a good convex \acrshort*{sdp} relaxation of the non-convex contact dynamics, and by encoding the hybrid problem using the graph structure presented in~\cite{marcucci2023shortest}, the use of convex relaxations enables us to simultaneously solve both the hybrid and non-convex parts of the of the problem as one convex optimization program.

%Today, planar pushing is typically solved with imitation learning~\cite{chiDiffusionPolicyVisuomotor2023a}, or in two steps with a sampling-based method~\cite{chengContactModeGuided2021a,chengContactModeGuided2022,pangGlobalPlanningContactRich2022,chavandafleInHandManipulationMotion2018} or a local motion planning method~\cite{doshiHybridDifferentialDynamic2020,lefebvreDifferentialFlatnessSliderPusher2023,zhouPushingRevisitedDifferential2019}, combined with a model-based control approach~\cite{hoganReactivePlanarNonprehensile2020,hoganFeedbackControlPusherSlider2020}.
%\aacomment{We can probably fold this into the intro.}

%Most existing methods are local, using either sampling~\cite{chengContactModeGuided2021a,chengContactModeGuided2022,pangGlobalPlanningContactRich2022,chavandafleInHandManipulationMotion2018} or \acrfull*{nlp}~\cite{doshiHybridDifferentialDynamic2020,posaDirectMethodTrajectory2014}.
%An advantage of these methods is that they can avoid explicitly reasoning about modes of the system, and provide useful plans for many tasks.
%However, local planners can be unreliable and may fail for tasks that require global reasoning.
%On the other hand, global methods exist, but are not quite effective. \aacomment{"effective" in what way?}
%Globally optimal plans can be achieved through the use of spatial \acrfull*{bb} methods, where the non-convex search space is partioned into smaller subsets, and the problem is solved through exhaustive enumeration \cite{koolenBalanceControlLocomotion2020}. 
%However, these methods suffer from poor scalability, as non-convexity is essentially replaced with increased combinatorial complexity.

%\tmcomment{Some relevant works:
%\begin{itemize}
%\item 
%Trajectory optimization~\cite{mordatch2012discovery,tassa2012synthesis}.
%As well as the contact implicit stuff~\cite{manchester2020variational}.
%But we should add more...
%\item Sampling based work by Pang and Terry~\cite{pang2023global}.
%\item Control through contact using mixed integer optimization.
%The work by Francois that you already cite, e.g.,~\cite{hoganFeedbackControlPusherSlider2020,hoganReactivePlanarNonprehensile2020}. 
%Prior to that, we worked on that topic for a few years using PWA models, see e.g.~\cite{marcucci2017approximate,marcucci2019mixed}.
%But also~\cite{aceituno2017simultaneous}.
%Also Mike Posa has worked on this recently~\cite{aydinoglu2022real}
%\item Some more or less random RL works~\cite{lillicrap2015continuous,gu2017deep,rajeswaran2017learning}.
%This uses RL on Anymal and works really well for quadrupeds~\cite{hwangbo2019learning}.
%RL for manipulation~\cite{andrychowicz2020learning,chen2022system}
%By Terry~\cite{yin2023rotating}
%\item This paper by Pete had some impressing planar pushing tasks~\cite{florence2022implicit}.
%\item 
%This is the paper I mentioned to you ealier~\cite{liu2023model}. Model is identified through data, then the NN is sparsified, and global MIQP is used for planning.
%\item 
%Suggestion by Russ~\cite{ma2023eureka}.
%\end{itemize}
%}

%With the recent advances in learning, optimization-based methods can play a fundamental role in generating large quantities of expect demonstrations. However, current methods for planning contact-rich tasks are not satisfactory... \bpgcomment{TODO Write this paragraph, if we think we should include it.}
%\aacomment{It may be worth framing this as "Another approach is learning based methods which have shown impressive performance. However, even in this context, effective global optimzation algorithms are still useful for both benchmarking the performance of the learned system and for training it."}
%This can be a problem for several reasons, but is especially an obstacle for learning-based pipelines where one seeks to generate expert demonstration data for imitation-learning policies, which might be desirable for their demonstrated robustness and output-feedback properties~\cite{chiDiffusionPolicyVisuomotor2023a}.
%\tmcomment{The connection to learning is nice, but it's a big leap. I would start a new paragraph for that. Maybe saying something like ``With the recent advances in learning, optimization methods can play a fundamental role in generating large quantities of expert demonstrations. However, etc etc''.}




\begin{comment}
\subsection{Planar Pushing}
and in~\cite{akellaPosingPolygonalObjects} a heuristic method for reorienting polygonal objects in the plane was proposed.

There has been a number of works on planar pushing using motion primitives~\cite{akellaPosingPolygonalObjects,chaiObjectRearrangementPlanar2022}.

\todo{Add related work}
%\tmcomment{Consider moving the paragraph on planar pushing here if you modify the intro to be more about control through contact in general. I do think of PP as a toy example, so I don't think that it's fundamental to explain immediately how people solve it.}
Today, planar pushing is typically solved with imitation learning~\cite{chiDiffusionPolicyVisuomotor2023a}, or in two steps with a sampling-based method~\cite{chengContactModeGuided2021a,chengContactModeGuided2022,pangGlobalPlanningContactRich2022,chavandafleInHandManipulationMotion2018} or a local motion planning method~\cite{doshiHybridDifferentialDynamic2020,lefebvreDifferentialFlatnessSliderPusher2023,zhouPushingRevisitedDifferential2019}, combined with a model-based control approach~\cite{hoganReactivePlanarNonprehensile2020,hoganFeedbackControlPusherSlider2020}.
\aacomment{We can probably fold this into the intro.}

The problem of planar pushing has gained much attention since the seminal work by Mason~\cite{masonMechanicsPlanningManipulator1986}.
Some early works include~\cite{goyalPlanarSlidingDry1991}, where Goyal et. al introduced the limit surface for modelling the interaction between the total frictional wrench and the motion of an object, or~\cite{lynchManipulationActiveSensing1992}, where Lynch introduced a simple approximation of the limit surface for use in feedback control for planar pushing, later used for an ad-hoc planning algorithm in~\cite{lynchStablePushingMechanics1996}.
\newacronym{ddp}{DDP}{Differential Dynamic Programming}
More recently, there has been several works on optimal planning and control for planar pushing tasks using the same limit surface approximation.
A hybrid \acrfull*{mpc} method is proposed for stabilizing a trajectory in~\cite{hoganFeedbackControlPusherSlider2020} and~\cite{hoganReactivePlanarNonprehensile2020}, and a local planning and control algorithm based on \acrfull*{ddp} is proposed in~\cite{doshiHybridDifferentialDynamic2020}.
A sampling-based planning method motion cones, an an extension of the limit surface, was presented in \cite{chavandafleInHandManipulationMotion2018}.


%Imitation-learning approaches demonstrate several impressive characteristics, such as output feedback and robustness to disturbances. However, they require demonstrations for training, which currently is an expensive data-gathering process executed by human operators.
%In principle, one can envision an imitation learning pipeline where a combination of model-based motion planning and control method provides optimal demonstrations, which are used to train a learned policy with the desirable characteristics as mentioned above.
%However, current motion-planning techniques are not well suited for such a pipeline: Sampling-based motion planning has the drawback of randomized plans, whereas local motion planning gets stuck in local minima.
%This motivates the search for a model-based motion planning algorithm which can provide globally optimal motion plans.
%\bpgcomment{Do we want a paragraph like this, mentioning the IM pipeline etc?}
%\subsection{Semidefinite Relaxations in Robotics}
%\tmcomment{Is this something that people do in planning? I know Luca Carlone has used some SDP stuff but mostly for localization. Maybe we can enlarge this to SDP relaxations in robotics?}
\end{comment}


==> sections/deprecated_vol_2/savva_related_works.tex <==
%!TEX root = ../root.tex

%\subsection{Control through contact}

% \bpgcomment{Focus here has been getting the structure right. For this whole section: Improve language, add more references.}

Approaches for planning through contact can generally be categorized into learning-based, search-based, and optimization-based methods.
% \tmcomment{I would pick ``planning through contact'' and avoid saying all the time ``planning and control through contact''}

\acrfull*{rl} and \acrfull*{bc} have proven very effective in tackling problems with contact dynamics.
\acrshort*{rl} has shown impressive robustness in quadruped locomotion~\cite{hwangbo2019learning, lee2020learning, siekmann2021sim}, and has been successfully applied to a variety of manipulation tasks in simulation~\cite{lillicrap2015continuous,rajeswaran2017learning}, real-world robotic manipulation~\cite{gu2017deep, pmlr-v87-kalashnikov18a}, and more recently 
% have shown great success 
with real-world dexterous hands \cite{andrychowicz2020learning, chen2022system, qi2023general, yin2023rotating}.
% One reason why RL through contact has proven particularly effective is because it abstracts low-level combinatorial decision making via sampling and averaging.
RL have proven particularly effective due to its ability to bypass the process of making low-level combinatorial contact decisions by using stochastic approximation schemes \cite{suh2022differentiable, suh2022bundled, lidec2022leveraging}.
% \aacomment{I don't know what this means.}
% \smcomment{i'm referencing Terry's work here to imply "RL does low-level better than opt-based-methods". will talk to him about how to phrase it better.}
% , but struggle with general long-horizon planning.
Though applicable to a variety of systems, these methods tend to require expensive training, careful curricula, and system-specific user-shaped reward functions.
% (with recent methods attempting to address these issues\cite{ma2023eureka} \smcomment{refs}).
\acrshort*{bc} methods have been successfully applied to planning and navigation~\cite{janner2022planning, sridhar2023nomad}, planar pushing~\cite{florence2022implicit}, and a variety of general manipulation tasks~\cite{chi2023diffusion, octo_2023, shafiullah2023bringing}.
These methods tend to require expensive expert demonstrations, often generated with teleoperation.
Our methodology can provide such expert near-optimal trajectories at a lower cost.

Sampling-based methods have also proven to be effective for planning through contact.
These methods tend to alternate between continuous trajectory optimization within the current mode and discrete sampling for the next mode.
Though in principle this facilitates global search, the inability to jointly search over discrete and continuous decisions makes finding optimal solutions nearly impossible.
Another key challenge is that the feasible contact configurations lie on lower-dimensional constrained manifolds, necessitating guided exploration in sampling.
Existing methods either assume the ability to sample from individual contact modes \cite{chengContactModeGuided2021a, chengContactModeGuided2022, vega2020asymptotically,chen2021trajectotree}, guide the search by estimating reachable sets in configuration space \cite{chavan-dafle2020planar, wu2020r3t}, or utilize a combination of smoothed contact models and custom contact samplers \cite{pangGlobalPlanningContactRich2022}.
The necessity for system-specific hand-crafted samplers makes using sampling-based methods difficult in practice.

% sampling distributions makes the practical use of sampling-based methods challenging.


% While they naturally enable global planning, the key challenge for these methods is that the feasible contact configurations lie on a lower-dimensional constrained manifolds, which require system-specific sampling distributions that can be challenging to obtain.

% These methods often offer a more global perspective compared to methods based on Nonlinear Programming (\acrshort{nlp}), enabling reasoning about tasks at a higher level. 
% However, sampling on constraint-manifolds poses challenges and may seem unnatural.

% Existing methods that either enumerate contact modes to guide the search have been employed for a variety of different non-prehensile tasks~\cite{chengContactModeGuided2021a,chengContactModeGuided2022}, or methods that use smoothed contact models to avoid reasoning explicitly about the contact modes have been employed to plan for dexterous hands and other contact-right manipulation~\cite{pangGlobalPlanningContactRich2022}.

% \bpgcomment{Add \cite{chavan-dafle2020planar} that use sampling-based methods to sample configurations on the motion cone}
% These methods are often in some sense more global than the methods based on \acrshort*{nlp}, and can reason about tasks at a more global level. However, sampling on constraint-manifolds is hard and seems unnatural.

% Optimization-based methods for planning through contact fall into two categories: contact-implicit and hybrid. \bpgcomment{In these two paragraphs it seems like we label all methods as either contact-implicit or MIP. But what about i.e. \cite{mordatch2012discovery}, would people label this as contact-implicit? I would think not?}
% \smcomment{that's the contact-invariant optimization paper; correct me if i'm wrong, contact-invariant / contact complementarity works fall under one idea: contact implicit opt, which write nonlinear constraints that consider for each possible contact mode at that timestep.}

Optimization-based methods broadly fall into two categories which differ in how the contact system is modeled. 
The first category are contact-implicit models, which model the contact as the solution set of a complementarity equation. 
These methods have the advantage of being amenable to traditional, smooth optimization techniques by either producing smooth approximations to the contact dynamics~\cite{mordatch2012discovery, tassa2012synthesis, tassa2014control, howell2022trajectory, chatzinikolaidis2021trajectory}, or directly operating on the complementarity formulation~\cite{posaDirectMethodTrajectory2014, sleiman2019contact, manchester2020variational, jinTaskDrivenHybridModel2022, wangContactImplicitPlanningControl2023}. 
While these methods have shown great performance in both locomotion and manipulation, they are inherently local and require a high-quality initial guess, which can be difficult to obtain\cite{wensing2023optimization}.
% Such guesses can be difficult to obtain in contact-rich problems with long horizons \aacomment{I need to put a citation here.}


% those that represent contact with nonlinear constraints using \acrfull{nlp}, and those that model contact combinatorially as discrete decisions using \acrfull{mip}.

% Contact-implicit methods formulate nonlinear constraints between system state and contact forces, solving the resulting optimization with \acrfull*{nlp}.
% These approaches either produce smooth approximations of contact dynamics\cite{mordatch2012discovery, tassa2012synthesis, tassa2014control, howell2022trajectory, chatzinikolaidis2021trajectory}, or employ the contact complementarity formulation \cite{posaDirectMethodTrajectory2014, sleiman2019contact, manchester2020variational, jinTaskDrivenHybridModel2022, wangContactImplicitPlanningControl2023}.
% Contact-implicit planning has shown great performance in both locomotion and manipulation, but it is inherently local and often requires a high-quality initial guess.


% Performance of \acrshort*{mip} solvers is dependent on the quality of 

% Hybrid methods plan for globally optimal trajectories by jointly optimizing over discrete contact modes and continuous robot motions, which are naturally solved with \acrfull*{mip}.

% which partition the sspace 
% with the search space is partitioned

% with globally 

% where globally optimal paths are attained by enumerating individual contact mode sequences
% mention branch and bound

% Hybrid methods plan for globally optimal trajectories by jointly optimizing over discrete contact modes and continuous robot motions.
% These are naturally solved with \acrfull*{mip}.
% These methods have shown success for relatively simple tasks, yet they suffer from poor scalability.
Hybrid methods plan globally optimal trajectories by jointly optimizing over discrete contact modes and continuous robot motions.
This optimization is naturally solved with \acrfull*{mip} and has been successfully applied to a variety of locomotion~\cite{ibanez2014emergence, aceituno2017simultaneous, koolenBalanceControlLocomotion2020} and manipulation tasks~\cite{aceituno-cabezasGlobalQuasiDynamicModel2020, hoganReactivePlanarNonprehensile2020}.
Common approaches often suffer from scalability issues, as the efficiency of \acrshort*{mip} is highly sensitive to the formulation of the discrete component of the planning problem.~\cite{marcucci2019mixed}
% 
% is dependent on the quality of the relaxation of the discrete contact modes constraints.

% Nonlinearities in the smooth dynamics within a contact mode, such as the ones associated with rotations and cross-products between contact points and forces, need to be handled too.
\acrshort*{mip} efficiency is also sensitive to the way that the nonlinearities in the smooth dynamics are handled.
% Nonlinearities in the smooth dynamics within a contact mode must be handled too.
A common approach is to produce a \acrfull*{pwa} approximation of the nonlinear dynamics, casting the problem as a \acrshort*{mip}~\cite{marcucci2019mixed}.
This approach has been applied to push-recovery~\cite{marcucci2017approximate}, planar pushing~\cite{hoganReactivePlanarNonprehensile2020}, and general manipulation tasks \cite{aceituno2017simultaneous, aydinoglu2022real}.
Although nonlinearity in the dynamics can be approximated arbitrarily well by using multiple linearization points and extra integer variables, the solve times of the resulting MIPs are exponential in the accuracy of this approximation (see, e.g.,~\cite{deits2014footstep}).
More recently, efficient task-specific \acrshort*{pwa} approximation have been obtained via learning ~\cite{hoganReactivePlanarNonprehensile2020, liu2023model}.
Yet another approach approximates smooth nonlinear dynamics with a difference of convex quadratic functions embedded into into SDP and QCQP relaxations~\cite{ponton2016convex}.
The authors then solve MIQCQP through contact in application to humanoid locomotion.
% In contrast, we produce different SDP relaxations of smooth nonlinear dynamics in conjunction with much tighter \acrshort*{mip} formulations.


Our method is most similar to this last category. In this work, we similarly produce an \acrshort*{sdp} approximation of the contact dynamics that is more compact than that of \cite{ponton2016convex}. Additionally, we depart from prior work by modelling the discrete choice of contact modes as an \acrshort*{spp} in a \acrshort*{gcs} which has seen success in producing substantially tighter convex relaxations of \acrshort*{mip}-based planning problems \cite{marcucci2023motionplanning}. The tightness of this formulation enables us to solve the entire problem as a single, large \acrshort*{sdp} followed by a cheap rounding solution using local methods. This is the first work to our knowledge to effectively use a single \acrshort*{sdp} to effectively solve the entire global motion planning problem.

% \smcomment{above: old}

% \smcomment{below: new}




% The second category models the contact system as a hybrid-dynamical system and so are known as hybrid models. The optimization method then plans trajectories by jointly optimizing over the discrete choice of contact modes and the continuous robot motions by solving a \acrfull*{mip}. These methods are able to plan globally by exploring the combinatorial many choices of the contact-mode and locations and have been successfully applied in a variety of both locomotion~\cite{ibanez2014emergence, aceituno2017simultaneous, koolenBalanceControlLocomotion2020}, and simple manipulations tasks such as push-recovery~\cite{marcucci2017approximate}, planar pushing~\cite{hoganReactivePlanarNonprehensile2020}, and others~\cite{aceituno2017simultaneous, aydinoglu2022real}. 


% % Solution methods for these models usually proceed by repeatedly solving convex, outer approximations of the original, discrete, non-convex optimization problems. The efficiency of these methods is therefore highly dependent on the ability to formulate both a good, convex approximation for the non-linear dynamics and the reliability of obtaining near-integer solutions in the relaxed problem. 
% % \smcomment{do we need this last paragraph? section already long}

% Many works have focused on the problem of generating good convex approximations to the dynamics, the most common of which is to produce a \acrfull*{pwa} approximation of the nonlinear dynamics, which have efficient \acrshort*{mip} formulations ~\cite{marcucci2019mixed}. Although nonlinearity in the dynamics can be approximated arbitrarily well by using multiple linearization points and additional integer variables, the solve times of the resulting MIPs are exponential in the accuracy of this approximation (see, e.g.,~\cite{deits2014footstep}).
% More recently, compact task-specific \acrshort*{pwa} approximation have been obtained via learning ~\cite{hoganReactivePlanarNonprehensile2020, liu2023model}.

% Another method for approximating the complex dynamics is based on the polynomial and semidefinite optimization literature \cite{posa2017balancing, blekherman2012semidefinite, lasserreMomentSOSHierarchy2018}. These formulations avoid the combinatorial blow up of \acrshort*{pwa} approximations by encoding the approximate dynamics as an \acrshort*{sdp}. The authors in \cite{ponton2016convex} use such a technique, providing both an \acrshort*{sdp} and \acrshort*{qcqp} approximation to the contact dynamics. As solving MISDPs are prohibitively expensive, the authors of that work resort to solving the planning problem as an MIQCQP.

% Our method is most similar to this last category. In this work, we similarly produce an \acrshort*{sdp} approximation of the contact dynamics that is more compact than that of \cite{ponton2016convex}. Additionally, we depart from prior work by modelling the discrete choice of contact modes as an \acrshort*{spp} in a \acrshort*{gcs} which has seen success in producing substantially tighter convex relaxations of \acrshort*{mip}-based planning problems \cite{marcucci2023motionplanning}. The tightness of this formulation enables us to solve the entire problem as a single, large \acrshort*{sdp} followed by a cheap rounding solution using local, methods. This is the first work to our knowledge to effectively use a single \acrshort*{sdp} to effectively solve the entire global motion planning problem.

% In this work, we blend the strengths of both methods. Beginning from the contact-implicit formulation of the system, we produce a tight, convex approximation of our contact dynamics by leveraging \acrfull*{sdp}. This formulation avoids the combinatorial blow up of the resulting optimization common in \acrshot*{pwa} formulations. This convex outer-approximation is then  

% This work falls into the category of hybrid methods. In contrast to prior work, we circumvent the exponential complexity of approximating the dynamics as a \acrfull*{pwa}

% Hybrid methods plan globally optimal trajectories by jointly optimizing over discrete contact modes and continuous robot motions.
% This optimization is naturally solved with \acrfull*{mip} and has been successfully applied to a variety of locomotion~\cite{ibanez2014emergence, aceituno2017simultaneous, koolenBalanceControlLocomotion2020} and manipulation tasks~\cite{aceituno-cabezasGlobalQuasiDynamicModel2020, hoganReactivePlanarNonprehensile2020}. 
% The efficiency of \acrshort*{mip} is dependent on the quality of the relaxation of the discrete contact modes constraints.
% Further relaxations are required to handle smooth nonlinearities in system dynamics, such as the ones associated with rotations and cross-products between contact points and forces.
% A common approach is to produce a \acrfull*{pwa} approximation of the nonlinear dynamics, which have efficient MIP formulations ~\cite{marcucci2019mixed}.
% This approach has been applied to push-recovery~\cite{marcucci2017approximate}, planar pushing~\cite{hoganReactivePlanarNonprehensile2020}, and general manipulation tasks \cite{aceituno2017simultaneous, aydinoglu2022real}.
% Although nonlinearity in the dynamics can be approximated arbitrarily well by using multiple linearization points and extra integer variables, the solve times of the resulting MIPs are exponential in the accuracy of this approximation (see, e.g.,~\cite{deits2014footstep}).
% More recently, efficient task-specific \acrshort*{pwa} approximation have been obtained via learning ~\cite{hoganReactivePlanarNonprehensile2020, liu2023model}.
% Yet another approach approximates smooth nonlinear dynamics with a difference of convex quadratic functions embedded into into SDP and QCQP relaxations~\cite{ponton2016convex}.
% The authors then solve MIQCQP through contact in application to humanoid locomotion.
% In contrast, we produce different SDP relaxations of smooth nonlinear dynamics in conjunction with much tighter \acrshort*{mip} formulations.
% % resulting in a MISDP and MIQCQP relaxation.
% % Yet another approach is to leverage convex relaxations of the nonlinear dynamics, in combination with \acrshort*{mip} which has been applied to locomotion in ~\cite{ponton2016convex}. \tmcomment{This seems very related to our approach? Might be worth emphasizing what we do differently?} \smcomment{working on it; anyone read that paper?}

% % \rtcomment{I think you are saying the right things, but perhaps missing the emphasis I would expect? the specific way that previous approaches struggled is by making a combinatorial piecewise approximation of the rotations; we use the SDP relaxations and show that they are tight.}
% % \smcomment{There are two relaxations happening here: discrete choices and rotation. In discrete perspective, most methods used big M integer relaxations(correct me Tobia if that's false), which are terribly lose; perspective machinery of gcs fixed that. for rotations, people discretized rotations or used mccormic envelopes. Your relaxation is more precise + tighter. I'd imagine you should put emphasis on both these things in discussing MICP literature}
% % \tmcomment{I added an extra sentence above. LMK if you like it.}
% % Yet another approach is to leverage convex relaxations of the nonlinear dynamics, in combination with \acrshort*{mip} which has been applied to locomotion in ~\cite{ponton2016convex}. \tmcomment{This seems very related to our approach? Might be worth emphasizing what we do differently?}

% Our method is close in spirit to the \acrshort*{mip} category, but is significantly more efficient.
% The contact transitions are modelled explicitly through a graph, and smooth dynamics nonlinearities are relaxed through an \acrshort*{sdp}.
% The resulting optimization problem is an SPP in GCS, whose rich structure can be exploited by highly effective methods based on convex optimization~\cite{marcucci2023shortest}.
% This enables us to tackle the combinatorial and the continuous components of the contact problems jointly through a unified convex optimization problem.

%Today, planar pushing is typically solved with imitation learning~\cite{chiDiffusionPolicyVisuomotor2023a}, or in two steps with a sampling-based method~\cite{chengContactModeGuided2021a,chengContactModeGuided2022,pangGlobalPlanningContactRich2022,chavandafleInHandManipulationMotion2018} or a local motion planning method~\cite{doshiHybridDifferentialDynamic2020,lefebvreDifferentialFlatnessSliderPusher2023,zhouPushingRevisitedDifferential2019}, combined with a model-based control approach~\cite{hoganReactivePlanarNonprehensile2020,hoganFeedbackControlPusherSlider2020}.
%\aacomment{We can probably fold this into the intro.}

%Most existing methods are local, using either sampling~\cite{chengContactModeGuided2021a,chengContactModeGuided2022,pangGlobalPlanningContactRich2022,chavandafleInHandManipulationMotion2018} or \acrfull*{nlp}~\cite{doshiHybridDifferentialDynamic2020,posaDirectMethodTrajectory2014}.
%An advantage of these methods is that they can avoid explicitly reasoning about modes of the system, and provide useful plans for many tasks.
%However, local planners can be unreliable and may fail for tasks that require global reasoning.
%On the other hand, global methods exist, but are not quite effective. \aacomment{"effective" in what way?}
%Globally optimal plans can be achieved through the use of spatial \acrfull*{bb} methods, where the non-convex search space is partioned into smaller subsets, and the problem is solved through exhaustive enumeration \cite{koolenBalanceControlLocomotion2020}. 
%However, these methods suffer from poor scalability, as non-convexity is essentially replaced with increased combinatorial complexity.

%\tmcomment{Some relevant works:
%\begin{itemize}
%\item 
%Trajectory optimization~\cite{mordatch2012discovery,tassa2012synthesis}.
%As well as the contact implicit stuff~\cite{manchester2020variational}.
%But we should add more...
%\item Sampling based work by Pang and Terry~\cite{pang2023global}.
%\item Control through contact using mixed integer optimization.
%The work by Francois that you already cite, e.g.,~\cite{hoganFeedbackControlPusherSlider2020,hoganReactivePlanarNonprehensile2020}. 
%Prior to that, we worked on that topic for a few years using PWA models, see e.g.~\cite{marcucci2017approximate,marcucci2019mixed}.
%But also~\cite{aceituno2017simultaneous}.
%Also Mike Posa has worked on this recently~\cite{aydinoglu2022real}
%\item Some more or less random RL works~\cite{lillicrap2015continuous,gu2017deep,rajeswaran2017learning}.
%This uses RL on Anymal and works really well for quadrupeds~\cite{hwangbo2019learning}.
%RL for manipulation~\cite{andrychowicz2020learning,chen2022system}
%By Terry~\cite{yin2023rotating}
%\item This paper by Pete had some impressing planar pushing tasks~\cite{florence2022implicit}.
%\item 
%This is the paper I mentioned to you ealier~\cite{liu2023model}. Model is identified through data, then the NN is sparsified, and global MIQP is used for planning.
%\item 
%Suggestion by Russ~\cite{ma2023eureka}.
%\end{itemize}
%}

%With the recent advances in learning, optimization-based methods can play a fundamental role in generating large quantities of expect demonstrations. However, current methods for planning contact-rich tasks are not satisfactory... \bpgcomment{TODO Write this paragraph, if we think we should include it.}
%\aacomment{It may be worth framing this as "Another approach is learning based methods which have shown impressive performance. However, even in this context, effective global optimzation algorithms are still useful for both benchmarking the performance of the learned system and for training it."}
%This can be a problem for several reasons, but is especially an obstacle for learning-based pipelines where one seeks to generate expert demonstration data for imitation-learning policies, which might be desirable for their demonstrated robustness and output-feedback properties~\cite{chiDiffusionPolicyVisuomotor2023a}.
%\tmcomment{The connection to learning is nice, but it's a big leap. I would start a new paragraph for that. Maybe saying something like ``With the recent advances in learning, optimization methods can play a fundamental role in generating large quantities of expert demonstrations. However, etc etc''.}




\begin{comment}
\subsection{Planar Pushing}
and in~\cite{akellaPosingPolygonalObjects} a heuristic method for reorienting polygonal objects in the plane was proposed.

There has been a number of works on planar pushing using motion primitives~\cite{akellaPosingPolygonalObjects,chaiObjectRearrangementPlanar2022}.

\todo{Add related work}
%\tmcomment{Consider moving the paragraph on planar pushing here if you modify the intro to be more about control through contact in general. I do think of PP as a toy example, so I don't think that it's fundamental to explain immediately how people solve it.}
Today, planar pushing is typically solved with imitation learning~\cite{chiDiffusionPolicyVisuomotor2023a}, or in two steps with a sampling-based method~\cite{chengContactModeGuided2021a,chengContactModeGuided2022,pangGlobalPlanningContactRich2022,chavandafleInHandManipulationMotion2018} or a local motion planning method~\cite{doshiHybridDifferentialDynamic2020,lefebvreDifferentialFlatnessSliderPusher2023,zhouPushingRevisitedDifferential2019}, combined with a model-based control approach~\cite{hoganReactivePlanarNonprehensile2020,hoganFeedbackControlPusherSlider2020}.
\aacomment{We can probably fold this into the intro.}

The problem of planar pushing has gained much attention since the seminal work by Mason~\cite{masonMechanicsPlanningManipulator1986}.
Some early works include~\cite{goyalPlanarSlidingDry1991}, where Goyal et. al introduced the limit surface for modelling the interaction between the total frictional wrench and the motion of an object, or~\cite{lynchManipulationActiveSensing1992}, where Lynch introduced a simple approximation of the limit surface for use in feedback control for planar pushing, later used for an ad-hoc planning algorithm in~\cite{lynchStablePushingMechanics1996}.
\newacronym{ddp}{DDP}{Differential Dynamic Programming}
More recently, there has been several works on optimal planning and control for planar pushing tasks using the same limit surface approximation.
A hybrid \acrfull*{mpc} method is proposed for stabilizing a trajectory in~\cite{hoganFeedbackControlPusherSlider2020} and~\cite{hoganReactivePlanarNonprehensile2020}, and a local planning and control algorithm based on \acrfull*{ddp} is proposed in~\cite{doshiHybridDifferentialDynamic2020}.
A sampling-based planning method motion cones, an an extension of the limit surface, was presented in \cite{chavandafleInHandManipulationMotion2018}.


%Imitation-learning approaches demonstrate several impressive characteristics, such as output feedback and robustness to disturbances. However, they require demonstrations for training, which currently is an expensive data-gathering process executed by human operators.
%In principle, one can envision an imitation learning pipeline where a combination of model-based motion planning and control method provides optimal demonstrations, which are used to train a learned policy with the desirable characteristics as mentioned above.
%However, current motion-planning techniques are not well suited for such a pipeline: Sampling-based motion planning has the drawback of randomized plans, whereas local motion planning gets stuck in local minima.
%This motivates the search for a model-based motion planning algorithm which can provide globally optimal motion plans.
%\bpgcomment{Do we want a paragraph like this, mentioning the IM pipeline etc?}
%\subsection{Semidefinite Relaxations in Robotics}
%\tmcomment{Is this something that people do in planning? I know Luca Carlone has used some SDP stuff but mostly for localization. Maybe we can enlarge this to SDP relaxations in robotics?}
\end{comment}


==> sections/response_to_reviewers.tex <==
\thispagestyle{empty} % No headers or footers on this page

\section*{Response to reviewers}

\subsection*{Summary of feedback in metareview:}
Here is the summary of the limitations/improvements from the metareview (strengths are left out):
\begin{quote}
\textbf{Limitations:}
\begin{itemize}
    \item  The coefficient of friction is assumed to be constant instead of dynamic.
    \item  The efficacy of the proposed approach diminishes when applied to objects with multiple faces, such as a T-shaped slider, due to increased planning times.
    \item The major concern is overstatement without validation, and the experiments do not contribute to the novelty and impact of the paper.
    \item The proposed method does not demonstrate a clear advantage over existing works.
\end{itemize}
\textbf{Improvements and clarifications:}
\begin{itemize}
    \item  Discuss how they are going to extend their approach to handle dynamic friction for more general and complex contact tasks.
    \item  Demonstrate the optimality and efficiency claims by comparing the generated planning with human demonstration and comparing with MIP or other methods in terms of computation time and trajectory.
    \item  Compare the proposed method with other strong baselines and demonstrate a clear advantage over existing works.
    \item  Clarify the values of the coefficients of friction for the box and T-shaped slider used in their experiments and how they were determined.
    \item  Discuss how this method could be adapted for fast motion planning of everyday objects, which might be considered to have an infinite number of faces
\end{itemize}
\end{quote}

\subsection*{High-level response to reviewers}
As our most immediate and high-level reaction to the reviews, we feel that perhaps the key point of the paper seems to have been somewhat misinterpreted, partially due to the application of the method on the specific problem of planar pushing. Specifically, the key message of the paper is proposing a novel method for global reasoning for contact-rich tasks, which substantially differs from all current methods in several ways:
\begin{itemize}
    \item It naturally solves both the discrete and continuous parts of the problem simultaneously and in a global way. This is in contrast to almost all existing methods, which either artificially decouple the discrete and continuous aspects, reason about the discrete and continuous parts at the same time but only do so locally, or rely on expensive global optimization algorithms which are not feasible to apply to problem instances of the size that we have (which includes mixed-integer approaches like \acrfull*{mincp}).
    \item Our method requires little to no tuning and almost always finds a feasible solution. This is in contrast to both local methods that require problem-specific heuristics for proposing initial guesses and (often) a significant tuning-effort to work well, as well as sampling-based methods that usually rely on a problem-specific and hand-crafted sampler. This is now clearly demonstrated in the new comparison section with a state-of-the-art baseline method in \cref{sec:comparison} that we have added as a response to the reviews. When planning for a non-convex slider geometry (the T-shape) our method is able to always find a solution, where the baseline fails in $88 \%$ of the instances, despite significant efforts to tune the baseline.
    \item Our method gives an objective way of quantifiying the quality of the trajectories through an upper bound on the global optimality gap, in contrast to local methods or sampling-based methods where this is not possible.
\end{itemize}

Further, we believe that the application to planar pushing has perhaps been a source of confusion in the review process.
In the original submitted draft we tried to highlight this in the abstract, the last paragraph of the introduction in \cref{sec:introduction}, and again in the conclusion/future work section in \cref{sec:conclusion}.
We have made some changes to make sure that this point is now properly conveyed, and will work on improving the clarity of this point in the final submission.
We certainly acknowledge that planar pushing in itself is a problem that can be solved for most practical purposes with i.e. learning-based methods, and we are definitely not trying to propose a better method for solving this problem in itself.
Rather, we choose to study our method on the problem of planar pushing, which only has the role as a suitable, initial, toy example that is still complex enough to capture the relevant hardness of contact-rich manipulation tasks.

For this reason, we also believe that some of the feedback we received regarding more complex friction modelling is outside the scope of the paper, as many of the most common robotics simulators do not even support friction models with dynamic friction coefficients, and also because the assumption of a constant friction coefficient is used by most comparable motion-planning methods for contact-rich manipulation planning that we are aware of.
However, we have still tried to address some of the feedback related to friction modelling it in the paper.

It is however correct that scaling is one of the main drawbacks of our approach at the moment. While we believe that there are several ways to remedy this (as we mention in the future works section in \cref{sec:conclusion}) and we have spent very little effort at this point in making the formulation more efficient, the current method as it is does not scale to realtime applications as pointed out by the reviewers and discussed in \cref{sec:conclusion}.
Yet, we believe that as the method currently stands in strong contrast to all comparable approaches, this strongly justifies the novelty of the paper.
In particular, we think that this point should be even more clear after highlighting its ability for joint global continuous/discrete reasoning compared to a state-of-the-art baseline for contact-rich planning in the comparison section in~\cref{sec:comparison} that we have added as a response to the reviews.


\subsection*{Overview of changes}
We have made several changes and improvements to the paper.
Most of the individual points from the reviewers feedback have been adressed by adding/adjusting parts of the paper to better highlight certain aspects of the work.
Most of these edits have an associated explanatory comment, which addresses the specific reviewer who gave the feedback.
All changes are highlighted in the text.
The biggest change in the paper is a comparison with a state-of-the-art baseline. List of changes:
\begin{itemize}
    \item Better emphasize that the main point of the paper is a novel motion-planning method that is capable of joint global discrete/continuous reasoning, and not a method tailored to solving planar pushing. This includes a few changes throughout the document.
    \item Reword the phrase "super-human", as it obscured the point we were trying to make.
    \item Specify drawbacks of mixed-integer-based approaches, and highlight how our method is more efficient.
    \item Address how more complex friction models may be incorporated.
    \item Add a subsection with a comparison (\cref{sec:comparison}) with a state-of-the-art baseline, which is chosen as a direct, contact-implicit trajectory-optimization method. The comparison highlights several of the advantages of our method, both through extensive testing and qualitative discussion.
    \item Add a figure that highlights some points from the comparison section.
    \item We added subsection titles in the experiments section in~\cref{sec:experiments} to clear up the structure after adding the comparison.
    \item State what friction model parameter values we use for the experiments, and how these were obtained
    \item Partly restructure the future work section to highlight the biggest drawback of the method (scaling) and how we are currently working on addressing it.
    \item Some typos and inconsistencies have been fixed throughout the document.
\end{itemize}

==> tables/experiment_results.tex <==
%!TEX root = ../root.tex

\begin{table}[htb]
	\centering
	\begin{tabular}{|c|c|c|} \hline
		Avg. tracking error & Avg. target error & Success Rate \\
  \hline
    X & X\% & X \%
    \\
  \hline
	\end{tabular}
	\caption{Experiment results. \bpgcomment{TODO}}
     \label{table:experiment_results}
\end{table}
